The All-Seeing Project: Towards Panoptic Visual Recognition and Understanding of the Open World

We present the All-Seeing (AS) project: a large-scale data and model for recognizing and understanding everything in the open world. Using a scalable data engine that incorporates human feedback and efficient models in the loop, we create a new dataset (AS-1B) with over 1 billion regions annotated with semantic tags, question-answering pairs, and detailed captions. It covers a wide range of 3.5 million common and rare concepts in the real world, and has 132.2 billion tokens that describe the concepts and their attributes. Leveraging this new dataset, we develop the All-Seeing model (ASM), a unified framework for panoptic visual recognition and understanding. The model is trained with open-ended language prompts and locations, which allows it to generalize to various vision and language tasks with remarkable zero-shot performance, including region-text retrieval, region recognition, captioning, and question-answering. We hope that this project can serve as a foundation for vision-language artificial general intelligence research. Models and the dataset shall be released at https://github.com/OpenGVLab/All-Seeing, and demo can be seen at https://huggingface.co/spaces/OpenGVLab/all-seeing.

==> tables/dataset_statistics_v2.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{0.8mm}    % table col width
\centering
\small
\begin{tabular}{@{}l|cccc|cc@{}}
\toprule
Dataset                 & \#Images & \#Regions & \#Concepts & \#Tokens & \begin{tabular}[c]{@{}c@{}}Open World\\ Location\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Open World\\ Semantic\end{tabular}        \\
\midrule
\emph{Image-Level}      &          &           &            &          &                                                                &                            \\
ImageNet-22K~\cite{deng2009imagenet}            & 15M      & $-$         & 22,000     & $-$        & $-$                                                              & \XSolidBrush               \\
Laion-5B~\cite{schuhmann2022laion5b}                & 5B       & $-$         & $-$          & 120.4B   &                                                                &                            \\
\midrule
\emph{Class-Agnostic}   &          &           &            &          &                                                                &                            \\
SA-1B~\cite{kirillov2023segment}                   & 11M      & 1.1B      & $-$          & $-$        & \textcolor{blue}{\Checkmark}                                   & $-$                          \\
\midrule
\emph{Region-Level}     &          &           &            &          &                                                                &                            \\
COCO~\cite{lin2014microsoft}                    & 0.1M     & 0.9M      & 80         & $-$        & \XSolidBrush                                                   & \XSolidBrush               \\
LVIS~\cite{gupta2019lvis}                    & 0.1M     & 1.5M      & 1,203      & $-$        & \XSolidBrush                                                   & \XSolidBrush               \\
Objects365~\cite{shao2019objects365}              & 0.6M     & 10.1M     & 365        & $-$        & \XSolidBrush                                                   & \XSolidBrush               \\
Open Images\cite{kuznetsova2020openimages}             & 1.5M     & 14.8M     & 600        & $-$        & \XSolidBrush                                                   & \XSolidBrush               \\
BigDetection~\cite{cai2022bigdetection}            & 3.5M     & 36.0M     & 600        & $-$        & \XSolidBrush                                                   & \XSolidBrush               \\
V3Det\cite{wang2023v3det}                   & 0.2M     & 1.5M      & 13,029     & $-$        & \XSolidBrush                                                   & \XSolidBrush               \\
Visual Genome\cite{krishna2017visualgenome}           & 0.1M     & 0.3M      & 18,136     & 35.2M    & \XSolidBrush                                                   & \XSolidBrush               \\
\rowcolor{mygray}
AS-2B(ours)             & \textbf{11M} \gbf{$\times$3}    & \textbf{2.2B} \gbf{$\times$61}     & \textbf{3.5M} \gbf{$\times$193}     & \textbf{132.2B} \gbf{$\times$3755}   & \textcolor{blue}{\Checkmark}  & \textcolor{blue}{\Checkmark}                \\
\bottomrule
\end{tabular}
\setlength{\abovecaptionskip}{0.15cm}
\caption{
    \textbf{Comparison with popular vision and vision-language datasets}. 
    ``\#'' denotes the number of something. We see that the proposed AS-2B dataset has a significantly larger data scale and diversity than prior region-level datasets.
}
\label{tab:dataset-comparisons}
\end{table}

==> tables/experiments_caption_auto.tex <==
\begin{table}[!t]
\footnotesize
\centering
\small
\begin{tabular}{@{}l|c|cc|cc|c|c@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Zero-Shot} & \multicolumn{2}{c|}{VG}         & \multicolumn{2}{c|}{RefCOCOg}   & \multicolumn{1}{c|}{Flickr30k} & \multicolumn{1}{c}{NoCap} \\
                       &                       & Meteor        & CIDEr          & Meteor        & CIDEr         & CIDEr                         & CIDEr                     \\ \midrule
Shikra-13B~\cite{chen2023shikra}             & \XSolidBrush                                          & $-$            & $-$              & $-$             & $-$              & 73.9                          & $-$                         \\
CoCa~\cite{yu2022coca}                   & \XSolidBrush                                          & $-$            & $-$              & $-$             & $-$                & $-$                             & \textbf{122.4}            \\
BLIP-2~\cite{li2023blip-2}                  & \XSolidBrush                                          & $-$             & $-$              & $-$             & $-$             & $-$                             & 121.0                     \\
InstructBLIP~\cite{instructblip}           & \XSolidBrush                                              & $-$             & $-$             & $-$              & $-$              & 82.8                          & 121.9                     \\
Kosmos-1~\cite{huang2023kosmos-1}               & \textcolor{blue}{\Checkmark}                       & $-$             & $-$             & $-$             & $-$                         & 67.1  &        $-$              \\
\midrule
GRiT~\cite{wu2022grit}                   & \XSolidBrush                                          & 17.1          & 142.0              & 15.2          & 71.6                     & $-$                             & $-$                         \\
SLR~\cite{yu2017slr}                    & \XSolidBrush                                          & $-$             & $-$              & 15.9          & 66.2           & $-$                                         & $-$                         \\
Kosmos-2~\cite{peng2023kosmos2}               & \textcolor{blue}{\Checkmark}                                           & $-$             & $-$              & 12.2          & 60.3                        & 66.7                          & $-$                         \\
\rowcolor{mygray}
ASM                    & \textcolor{blue}{\Checkmark}                                           & 12.6              & 44.2               & 13.6          & 41.9               & 77.9                          & 104.8                     \\
\rowcolor{mygray}
ASM-FT                 & \XSolidBrush                                          & \textbf{18.0} & \textbf{145.1} & \textbf{20.8} & \textbf{103.0}         & \textbf{87.7}                 & 117.2                     \\ \bottomrule
\end{tabular}
\caption{
\textbf{Quantitative results on image and region-level caption task.} \todo{check the table}}
\label{table:caption-automatic-evaluation}
\end{table}

==> tables/experiments_caption_auto_old.tex <==
\begin{table}[!t]
\footnotesize
\setlength{\tabcolsep}{1pt}
\centering
\small
\begin{tabular}{@{}l|c|cc|cc|cc|c|c@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Zero-Shot} & \multicolumn{2}{c|}{VG}         & \multicolumn{2}{c|}{RefCOCOg}   & \multicolumn{2}{c|}{COCO Caption} & \multicolumn{1}{c|}{Flickr30k} & \multicolumn{1}{c}{NoCap} \\
                       &                       & Meteor        & CIDEr          & Meteor        & CIDEr          & BLEU-4         & CIDEr          & CIDEr                         & CIDEr                     \\ \midrule
UniPerceiver-V2~\cite{li2023uni}        & \XSolidBrush                                          & $-$             & $-$              & $-$             & $-$              & 35.4           & 116.9          & $-$                            & $-$                         \\
VisionLLM~\cite{wang2023visionllm}              & \XSolidBrush                                          & $-$            & $-$             & $-$            & $-$             & 32.1           & 114.2          & $-$                             & $-$                        \\
Shikra-13B~\cite{chen2023shikra}             & \XSolidBrush                                          & $-$            & $-$              & $-$             & $-$              & $-$              & 117.5          & 73.9                          & $-$                         \\
CoCa~\cite{yu2022coca}                   & \XSolidBrush                                          & $-$            & $-$              & $-$             & $-$              & 40.9           & 143.6          & $-$                             & \textbf{122.4}            \\
BLIP-2~\cite{li2023blip-2}                  & \XSolidBrush                                          & -             & -              & -             & -              & \textbf{43.5}  & \textbf{145.2} & -                             & 121.0                     \\
InstructBLIP~\cite{instructblip}           & \XSolidBrush                                          & -             & -              & -             & -              & -              & -              & 82.8                          & 121.9                     \\
Kosmos-1~\cite{huang2023kosmos-1}               & \textcolor{blue}{\Checkmark}                                           & -             & -              & -             & -              & -              & 84.7           & 67.1                          & -                         \\
\midrule
GRiT~\cite{wu2022grit}                   & \XSolidBrush                                          & 17.1          & 142.0              & 15.2          & 71.6              & -              & -              & -                             & -                         \\
SLR~\cite{yu2017slr}                    & \XSolidBrush                                          & -             & -              & 15.9          & 66.2           & -              & -              & -                             & -                         \\
Kosmos-2~\cite{peng2023kosmos2}               & \textcolor{blue}{\Checkmark}                                           & -             & -              & 12.2          & 60.3           & -              & -              & 66.7                          & -                         \\
\rowcolor{mygray}
ASM                    & \textcolor{blue}{\Checkmark}                                           & 12.6              & 44.2               & 13.6          & 41.9           & 31.6           & 117.3          & 77.9                          & 104.8                     \\
\rowcolor{mygray}
ASM-FT                 & \XSolidBrush                                          & \textbf{18.0} & \textbf{145.1} & \textbf{20.8} & \textbf{103.0} & 39.2           & 136.9          & \textbf{87.7}                 & 117.2                     \\ \bottomrule
\end{tabular}
\caption{
\textbf{Quantitative results on image and region-level caption task.} \todo{check the table}}
\label{table:caption-automatic-evaluation}
\end{table}

==> tables/experiments_vqa_human.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{@{}crrrrr@{}}
\toprule
      & Total Questions & LLaVA~\cite{liu2023llava} & MiniGPT4~\cite{zhu2023minigpt-4} & ASM & Unanswerable \\ \midrule
Ratio & xxx             & xxx   & xxx      & xxx & xxx          \\ \bottomrule
\end{tabular}
\caption{Human votes on the answers which is best fit to the visual questions.}
\label{table:vqa-human-evaluation}
\end{table}

==> tables/region_valid_ratio.tex <==


\begin{tabular}{l|c|c|c|c|c}
\toprule
Region Type & LLMs   & BLIP-2  & InternImage & EVA  & GLIP      \\ \midrule
Tiny        & 18.6\% & 23.6\% & 71.3\%  & 77.9\% & $-$    \\
Small       & 25.3\% & 34.7\% & 62.9\% & 72.0\% & 76.5\% \\
Medium      & 37.5\% & 51.9\% & 61.5\% & 65.6\% & 67.3\% \\
Large       & 40.2\% & 55.2\% & 61.4\% & 61.6\% & 64.4\% \\
Xlarge      & 45.0\% & 58.9\% & 62.0\% & 60.2\% & 65.1\% \\
Huge        & 52.6\% & 69.0\% & 68.5\%  & 60.1\% & 69.9\% \\
All         & 40.4\% & 53.9\% & 62.5\%  & 65.5\% & 66.5\% \\ \bottomrule
\end{tabular}
